Sequential Joint Shape and Pose Estimation of Vehicles with Application to Automatic Amodal Segmentation Labeling

Shape and pose estimation is a critical perception problem for a self-driving car to fully understand its surrounding environment. One fundamental challenge in solving this problem is the incomplete sensor signal (e.g., LiDAR scans), especially for faraway or occluded objects. In this paper, we propose a novel algorithm to address this challenge, which explicitly leverages the sensor signal captured over consecutive time: the consecutive signals can provide more information about an object, including different viewpoints and its motion. By encoding the consecutive signals via a recurrent neural network, not only our algorithm improves the shape and pose estimates, but also produces a labeling tool that can benefit other tasks in autonomous driving research. Specifically, building upon our algorithm, we propose a novel pipeline to automatically annotate high-quality labels for amodal segmentation on images, which are hard and laborious to annotate manually. Our code and data will be made publicly available.

==> dump.tex <==
%Our framework consists of a feature encoder $f(\cdot)$ that extracts shared features for shapes and poses directly from the current point cloud measurement $Z_t$, a Gated Recurrent Unit (GRU) to fuse current features with those extracted from $Z_{1:t-1}$, a shape decoder $g_{\text{shape}}(\cdot)$ to infer the complete point cloud shape $X_t$, and a pose decoder $g_{\text{pose}}(\cdot)$ to infer the pose $T_t$. 

%We adopt the point cloud encoder architecture from Point Completion Network (PCN) \cite{pcn}, which consists of two stacked PointNet layers \cite{pointnet}. The fusion network is a single layer GRU that aggregates the previous state and the current input into a hidden state $h_t$ of dimension 1024. The pose decoder is a three-hidden-layer Multi-layer Perceptron (MLP) of size $1024\rightarrow512\rightarrow512\rightarrow3$, which predicts the planar translation and yaw angle $\theta$. The shape decoder follows the coarse decoder from PCN \cite{pcn}, which is an MLP of size $1024\rightarrow1024\rightarrow3N$, mapping the hidden state $h_t$ to a fixed-length $N=2048$ point cloud.

%First, we preprocess the point cloud measurement $Z_t$ by demeaning or shifting the measurement by its mean $\bar{Z}_t$, and bringing the object amodal center closer to the origin:

%That is, we will be making estimation using the updated hidden state $h_t$, rather than just $f_t$: $h_t$ has fused all available measurements $Z_{1:t}$. %prediction is made from the hidden state $h_t$ that has fused all available measurements $Z_{1:t}$.
%The hidden state $h_t$ represents the state at time $t$ and is updated recursively through the GRU module \cite{GRU} as new measurements are received over time:

%Utilizing information from all past measurements provides more information to produce richer features, which will in turn benefit the eventual shape and pose estimation. This improvement, however, does not come for free, as the point cloud measurements $Z_{1:t}$ are in different coordinate frames. Extracting a meaningful and powerful representation $h_t$ from $Z_{1:t}$ thus requires measurements $Z_{1:t}$ to be aligned and fused appropriately. While the aforementioned demeaning step also serves to bring measurements to the same coordinate frame in the point-cloud level, it is far from perfect, because the mean of a partial point cloud measurement does not align with the true center of the complete shape. Moreover, demeaning does not align the orientation of the points. Thus, the GRU fusion block must also learn to correct the alignment error at the feature level and fuse each measurement appropriately.
